Safe and Verified Gomory Mixed Integer Cuts in a Rational MIP Framework

This paper is concerned with the exact solution of mixed-integer programs (MIPs) over the rational numbers, i.e., without any roundoff errors and error tolerances. Here, one computational bottleneck that should be avoided whenever possible is to employ large-scale symbolic computations. Instead it is often possible to use safe directed rounding methods, e.g., to generate provably correct dual bounds. In this work, we continue to leverage this paradigm and extend an exact branch-and-bound framework by separation routines for safe cutting planes, based on the approach first introduced by Cook, Dash, Fukasawa, and Goycoolea in 2009. Constraints are aggregated safely using approximate dual multipliers from an LP solve, followed by mixed-integer rounding to generate provably valid, although slightly weaker inequalities. We generalize this approach to problem data that is not representable in floating-point arithmetic, add routines for controlling the encoding length of the resulting cutting planes, and show how these cutting planes can be verified according to the VIPR certificate standard. Furthermore, we analyze the performance impact of these cutting planes in the context of an exact MIP framework, showing that we can solve 21.5% more instances and reduce solving times by 26.8% on the MIPLIB 2017 benchmark test set.

==> certificate-overhead.tex <==
\small{
   \sisetup{round-mode=places,round-precision=1,table-number-alignment=right,table-format=2.1}
   \begin{tabular*}{\textwidth}{l@{\;\extracolsep{\fill}}llll}%{l@{\;\extracolsep{\fill}}rrrr}
      \toprule
      & \multicolumn{4}{c}{time [s]} \\
      \cmidrule(r){2-5}
      & solving                 & completion & checking & total \\
      \midrule
      Baseline          & 621.5                   & -          &  -       & 621.5 \\
      With verification & 914.4                   & 25.73      & 40.10    & 980.2 \\
      \midrule
      Overhead          & \overhead{914.4}{621.5} & -          & -        & \overhead{980.23}{621.5} \\
      \bottomrule
   \end{tabular*}
}


==> gapclosed.tex <==
% \begin{tabular}{lrrrr}
% \toprule
% {} & ClGap\_mean & ClGapRoot\_mean & ClGap\_meanQ & ClGapRoot\_meanQ \\
% Settings     &            &                &             &                 \\
% \midrule
% inter-noenc  &      0.573 &          0.197 &       1.000 &           1.000 \\
% inter-nosepa &      0.546 &          0.083 &       0.952 &           0.420 \\
% mediumden    &      0.606 &          0.197 &       1.059 &           0.997 \\
% reduced      &      0.620 &          0.141 &       1.082 &           0.715 \\
% reduced-cuts &      0.719 &          0.261 &       1.255 &           1.321 \\
% \bottomrule
% \end{tabular}


\begin{tabular}{lrrrrr}
   \toprule
   {}              & \nocuts & \safegmi & \enc  & \fpred & \fpcuts \\
   \midrule
   gap closed root & -       & 0.150    & 0.152 & -      & 0.161   \\
   gap closed tlim & 0.485   & 0.580    & 0.585 & 0.543  & 0.653   \\
   \bottomrule
\end{tabular}


==> oneoptimal_agg.tex <==

\begin{table}[t]
   \small{
     \caption{Comparison of original and new framework with presolving and primal heuristics disabled} %). Column ``dbtime'' shows the shifted geometric mean of timee spent in safe dual bounding.}
     \medskip
 
      \label{oldvsnew-avg}
      \sisetup{round-mode=places,round-precision=1}
      \begin{tabular*}{\textwidth}{lllll}
      \toprule
       {setting}      & {solved} & {time (rel)}  & {nodes (rel)}& {exlptime} \\
      \midrule
      no cuts         &       42 &  825.1        & 9512.6       & 47.7  \\
      cuts            &       44 &  655.4 (0.79) & 4905.0 (0.52)& 74.1  (1.55)\\
      cuts+approx     &       47 &  610.5 (0.74) & 5004.6 (0.53)& 45.0  (0.94) \\
      \midrule
      \end{tabular*}
      \vspace*{-1.2em}
   }
  \end{table}

==> runtime-fpcuts.tex <==
\begin{tabular}{lrrlrlrr}
   \toprule
           &        &         &       & \multicolumn{3}{c}{time [s]}                 \\
   \cmidrule(lr){5-7}
   setting & solved & nodes   & (rel) & total                        & (rel) & LP    \\
   \midrule
   \fpred  & 164    & 32741.6 & 1.00  & 695.29                       & 1.00  & 378.7 \\
   \fpcuts & 203    & 12604.8 & 0.38  & 451.12                       & 0.65  & 233.1 \\
   \bottomrule
\end{tabular}

==> runtime-safecuts.tex <==
% \begin{tabular}{lrrrrr}
%    \toprule
%    setting & size & solved & time & nodes & exlp time \\
%    \midrule
%    no cuts   &     154 &      128 &            895.2 &             12639.7 &                 71.7 \\
%    safe cuts    &     154 &      122 &            887.6 &              6118.2 &                120.1 \\
%    cuts + encoding length      &     154 &      141 &            811.5 &              7285.4 &                 76.52 \\
%    cuts + weakened &     154 &      127 &            890.7 &              6887.1 &                111.1 \\
%    \bottomrule
%    \end{tabular}

% \begin{tabular}{lrrrrrrrr}
%    \toprule
%    settings & size & solved & time & nodes & t exlp  & t exlp fail & n exlp & nfails exlp \\
%    \midrule
%    \nocuts   &     154 &      128 &            895.17 &             12639.7 &                  71.7 &                       0.0 &                   567.0 &                     0.0 \\
%    \safegmi  &     154 &      122 &            887.57 &              6118.2 &                 120.1 &                       4.7 &                   378.0 &                     5.1 \\
%    \enc      &     154 &      141 &            811.53 &              7285.4 &                  76.5 &                       0.3 &                   402.1 &                     0.4 \\
%    \bottomrule
% \end{tabular}

% \begin{tabular}{lrrrrrrr}
%    \toprule
%    & solved & Time & rel & Nodes & rel & ExLP t\/call & LP t\/call \\
%    Settings     &     & &     &                   &                     &               &             \\
%    \midrule      
%    \nocuts &      131 &            853.48 &   1.00   &       10793.9 &  1.00  &    1.1590 &      1.1022 \\
%    \safegmi  &      125 &            852.69 &  0.99  &          5552.7 & 0.51 &      1.4153 &      1.1136 \\
%    \enc    &      144 &            767.04 &    0.90  &        6358.4 &   0.59 &    1.2508 &      1.1270 \\
%    \bottomrule
% \end{tabular}

\begin{tabular}{lrrlrlrr}
   \toprule
   % AG: suggestion for new headers, also in next table
            &        &         &       & \multicolumn{4}{c}{time [s]}                        \\
   \cmidrule(lr){5-8}
   setting  & solved & nodes   & (rel) & total                        & (rel) & exLP & fpLP  \\
   %& solved & Time & rel & Nodes & rel & ExLP  & LP \\
   %setting     &     & &     &                   &                     &               &             \\
   \midrule
   \nocuts  & 130    & 20106.5 & 1.00  & 1121.06                      & 1.00  & 7.1  & 324.0 \\
   \safegmi & 152    & 9867.5  & 0.49  & 914.26                       & 0.82  & 18.7 & 216.8 \\
   \enc     & 158    & 9952.9  & 0.5   & 820.69                       & 0.73  & 11.1 & 209.5 \\
   \bottomrule
\end{tabular}


